SEntNet: Source-aware Recurrent Entity Network for Dialogue Response Selection

Dialogue response selection is an important part of Task-oriented Dialogue Systems (TDSs); it aims to predict an appropriate response given a dialogue context. Obtaining key information from a complex, long dialogue context is challenging, especially when different sources of information are available, e.g., the user's utterances, the system's responses, and results retrieved from a knowledge base (KB). Previous work ignores the type of information source and merges sources for response selection. However, accounting for the source type may lead to remarkable differences in the quality of response selection. We propose the Source-aware Recurrent Entity Network (SEntNet), which is aware of different information sources for the response selection process. SEntNet achieves this by employing source-specific memories to exploit differences in the usage of words and syntactic structure from different information sources (user, system, and KB). Experimental results show that SEntNet obtains 91.0% accuracy on the Dialog bAbI dataset, outperforming prior work by 4.7%. On the DSTC2 dataset, SEntNet obtains an accuracy of 41.2%, beating source unaware recurrent entity networks by 2.4%.

==> notations.tex <==
%!TEX root = 00-scai19-main.tex
\begin{table}[h]
% \vspace*{-0.25\baselineskip}
\setlength{\tabcolsep}{1pt}
\centering
\caption{Notation used in the paper.}\label{tab:notations}
\begin{tabular}{lp{6.25cm}}
\toprule
{\bfseries Symbol} &  {\bfseries Glossary}\\
\midrule
%%%%  Sets
$\mathbb{U}$ & Set of user utterances\\
$\mathbb{S}$ & Set of system responses\\
$\mathbb{B}$ & Set of retrieved results \\
%%%%  Objects
$u, s, b$ & A user utterance, system response, retrieved result\\
$\Source$ & Source of information \\
${k}_l, {v}_l$ & $l$-{th} slot ${k}_l$ and its corresponding value ${v}_l$\\
$\psi_{\Theta}$ & Dialogue selection model parameterized by $\Theta$ \\
$\mathbb{R}^{d}$ & Vector space with $d$ dimension\\
% $\sigma$ & Sigmoid function \todo{Do we need this?} \\
% $\phi$ & ReLU function \todo{Do we need this?} \\
%%%% Vectors
${w}_{x}^i$ & Embedding vector of $x$-{th} word of $i$-{th} utterance \\
$e_i$ & Embedding vector of $i$-{th} utterance \\
$q$ & Embedding vector of query $u_t$\\
${f}_x$ & Vector of learnable mask at position $x$ \\
$\tilde{h}_j^i$, ${h_j^i}$ & Vector of hidden state $\tilde{h}_j^i$ and its normalization ${h_j^i}$ of $j$-{th} entity in the $i$-{th} utterance \\
$h_j$ & Vector of hidden state $h_j$ of $j$-{th} entity\\
$z$ & Vector of sum of all hidden states\\
$y$ & Predicted distribution of response candidates \\
$\hat{y}$ & True distribution of response candidates \\
%%%% Scalar
% $p_j$ & The weight for the $j^{th}$ state \todo{Do we need this?} \\
$c$ & Number of all candidate responses \\
$d$ & Number of embedding dimensions \\
$l$ & Number of the required \textit{slots} \\
$m$ & Number of all memory blocks \\
$n$ & Number of all utterances \\
$\lambda$ & Number of retrieved results \\
$t$ & Index of the current dialogue turn \\
% $x$ & An index of the current word in an utterance \todo{Do we need this?} \\ 
%%%% Matrices
$E$ & Matrix of word embeddings for $\mathbb{U}$\\
%  $G, V, W, L, H$ & Learnable matrices \todo{do we need to claim them?} \\ 
\bottomrule
\end{tabular}
\vspace*{-0.5\baselineskip}
\end{table}

